A Q-learning Control Method for a Soft Robotic Arm Utilizing Training Data from a Rough Simulator

It is challenging to control a soft robot, where reinforcement learning methods have been applied with promising results. However, due to the poor sample efficiency, reinforcement learning methods require a large collection of training data, which limits their applications. In this paper, we propose a Q-learning controller for a physical soft robot, in which pre-trained models using data from a rough simulator are applied to improve the performance of the controller. We implement the method on our soft robot, i.e., Honeycomb Pneumatic Network (HPN) arm. The experiments show that the usage of pre-trained models can not only reduce the amount of the real-world training data, but also greatly improve its accuracy and convergence rate.

==> sections/disscussion.tex <==
\section{discussion and future works}

%Because our simulation model is relatively simple, and there are factors such as gravity in our experiments, our model based on PCC is very inaccurate. The experiments in this paper indicate that the pre-training in the simulation based on a simple and inaccurate model can also greatly improve the performance of the controller. We conjecture that this may be because the state definition adopted by our Q-learning method is only related to the pose of the goal and the pose of the tip of the arm, and is not related to the posture of the arm, the air pressure of the arm, and so on. Therefore, it is only necessary to ensure that when the tip of the arm in the simulation is in a similar pose to the tip of the arm in reality, the response of the two arms to the same actuation change is similar. And there is no need to ensure that the mapping from the actuation space to the task space is accurate. However, this conjecture has not yet been verified by any experiment. In future, we may further explore the causes of this phenomenon and propose a theory to explain it. In addition, in future, we will try to use more accurate simulation models to improve our pre-training performance.

The Q-learning method implemented in this work can be regarded as a special case of the dyna algorithm. As long as the model can be updated in real-time, and the Q table is updated based on the model during the point-to-point task, the Q-learning method implemented in this work can be upgraded to a dyna algorithm. The realization of the dyna algorithm will reduce the requirements for the model of the environment in which the soft arm is located and the objects it interacts with, so that the controller can be used in more applications scenes, especially in unstructured environments. In future, we may implement the dyna algorithm to improve the controller implemented in this work.

